From Dense to Sparse: Morton-Ordered Sparse Mapping for Efficient 3D Mesh Generation

Unified 3D understanding and generation require compact sequences preserving spatial structure. Dense grids yield long sequences, while serialization can separate spatial neighbors. We propose Sparse Proximity Aware Compression (SPAC), a shared sparse SDF vocabulary combining sparse encoding with reversible spatial merging. A Sparse SDF VQ-VAE quantizes near-surface features while retaining explicit coordinates, using reconstruction supervision for surface fidelity and detail. 3D Byte-Pair Encoding (3D-BPE) merges recurring face-adjacent patterns using relative offsets before serialization. Macro tokens expand exactly into leaf tokens and coordinates. After Morton serialization, a shared LLM reads geometry for captioning and predicts tokens that decode into meshes for text-conditioned generation. With fixed geometry, architecture, and band width in voxels, sparse encoder cost grows approximately quadratically with resolution. 3D-BPE reduces mean complete LLM sequence length by 45.4 percent, including coordinates, text, and control tokens. SPAC achieves strong results in both 3D captioning and text-conditioned mesh generation. Ablations show gains over leaf tokens and Morton 1D-BPE in both tasks. The project page at https://yangjj007.github.io/spac/ .

==> preamble.tex <==
% Additional packages and settings for RAVEC.
\usepackage{mathtools}
\usepackage{array}
\usepackage{longtable}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{placeins}
\usepackage{wrapfig}
\usepackage{xurl}

\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}

% Give in-text figures room to move while keeping paragraphs at natural spacing.
\renewcommand{\topfraction}{0.85}
\renewcommand{\bottomfraction}{0.8}
\renewcommand{\textfraction}{0.12}
\renewcommand{\floatpagefraction}{0.7}
\setcounter{topnumber}{3}
\setcounter{totalnumber}{5}
\setlength{\textfloatsep}{14pt plus 3pt minus 2pt}
\setlength{\intextsep}{12pt plus 3pt minus 2pt}
\setlength{\emergencystretch}{1em}

\newcommand{\cmark}{\textcolor{black}{\ding{51}}}
\newcommand{\xmark}{\textcolor{red}{\ding{55}}}
% Algorithm text stays black; only selected formulas receive pale backgrounds.
\definecolor{algdirbg}{RGB}{252,231,229}
\definecolor{algcreditbg}{RGB}{229,239,251}
\definecolor{algallocbg}{RGB}{255,240,214}
\definecolor{backbonerow}{gray}{0.94}
% Paint the whole row, including tabular*'s stretched column gaps.
\makeatletter
\newcommand{\shadebackbonerow}{\noalign{%
  \begingroup\color{backbonerow}%
  \hrule height\dimexpr\ht\@arstrutbox+\dp\@arstrutbox\relax
  \endgroup
  \vskip-\dimexpr\ht\@arstrutbox+\dp\@arstrutbox\relax}}
\makeatother
\newcommand{\algcomment}[1]{\hfill\mbox{\footnotesize\color{black}\(\triangleright\)~#1}}
\newcommand{\alghl}[2]{\begingroup\setlength{\fboxsep}{1.2pt}%
  \colorbox{#1}{\strut\ensuremath{\color{black}#2}}\endgroup}

% Use genuine equation tags so every number aligns with the column edge.
% Keep the existing wrappers and label arguments for the method equations.
\newenvironment{boxedEquation}[1]{%
  \begin{equation}\label{#1}%
}{%
  \end{equation}%
}

% Align the formula rows internally; amsmath places the number at the edge.
\newenvironment{alignedEquation}[1]{%
  \begin{equation}\label{#1}%
  \begin{aligned}%
}{%
  \end{aligned}%
  \end{equation}%
}

% Group definitions with a left brace and the same standard equation tag.
\newenvironment{bracedEquation}[1]{%
  \begin{equation}\label{#1}%
  \left\{\begin{aligned}%
}{%
  \end{aligned}\right.%
  \end{equation}%
}

